Higher order QCD corrections in exclusive charmless B decays

We discuss exclusive charmless B decays within the Standard Model of particle physics. In particular, we consider hadronic two-body decays as B -> pi pi and perform a conceptual analysis of heavy-to-light form factors which encode the strong interaction effects in semi-leptonic decays as B -> pi l nu. Concerning the hadronic decays we compute NNLO QCD corrections which are particularly important with respect to strong interaction phases and hence direct CP asymmetries. We present results for the imaginary part of the topological tree amplitudes and a partial calculation of the real part of the amplitudes which is technically more involved. In our conceptual analysis of the QCD dynamics in heavy-to-light transitions we consider form factors between non-relativistic bound states. We perform a NLO analysis and compute the so-called soft-overlap contribution which is calculable in our set-up. As a byproduct of our analysis, we calculate leading-twist light-cone distribution amplitudes for non-relativistic bound states which can be applied for B_c or eta_c mesons.

==> abstract_spires.tex <==
We discuss exclusive charmless B decays within the Standard Model of
particle physics. In particular, we consider hadronic two-body
decays as B -> pi pi and perform a conceptual analysis of
heavy-to-light form factors which encode the strong interaction
effects in semi-leptonic decays as B -> pi l nu.

Concerning the hadronic decays we compute NNLO QCD corrections which
are particularly important with respect to strong interaction phases
and hence direct CP asymmetries. We present results for the
imaginary part of the topological tree amplitudes and a partial
calculation of the real part of the amplitudes which is technically
much more involved.

In our conceptual analysis of the QCD dynamics in heavy-to-light
transitions we consider form factors between non-relativistic bound
states. We perform a NLO analysis and compute the so-called
soft-overlap contribution which is calculable in our set-up. As a
byproduct of our analysis, we calculate leading-twist light-cone
distribution amplitudes for non-relativistic bound states which can
be applied for the description of B_c or eta_c mesons.

